A Distributed Auctioneer for Resource Allocation in Decentralized Systems

In decentralized systems, nodes often need to coordinate to access shared resources in a fair manner. One approach to perform such arbitration is to rely on auction mechanisms. Although there is an extensive literature that studies auctions, most of these works assume the existence of a central, trusted auctioneer. Unfortunately, in fully decentralized systems, where the nodes that need to cooperate operate under separate spheres of control, such central trusted entity may not exist. Notable examples of such decentralized systems include community networks, clouds of clouds, cooperative nano data centres, among others. In this paper, we make theoretical and practical contributions to distribute the role of the auctioneer. From the theoretical perspective, we propose a framework of distributed simulations of the auctioneer that are Nash equilibria resilient to coalitions and asynchrony. From the practical perspective, our protocols leverage the distributed nature of the simulations to parallelise the execution. We have implemented a prototype that instantiates the framework for bandwidth allocation in community networks, and evaluated it in a real distributed setting.

==> title.tex <==

% paper title
\title{A Distributed Auctioneer for Resource Allocation in Decentralized Systems}

% author names and affiliations
\author{
	\IEEEauthorblockN{ 
		Amin M. Khan\IEEEauthorrefmark{1}\IEEEauthorrefmark{2},
		Xavier Vilaça\IEEEauthorrefmark{1},
		Luís Rodrigues\IEEEauthorrefmark{1},
		Felix Freitag\IEEEauthorrefmark{2},
	}
	
	\IEEEauthorblockA{ 
		\IEEEauthorrefmark{1}
		Instituto Superior Técnico, Universidade de Lisboa. INESC-ID Lisboa. Lisbon, Portugal
		\\\{amin.khan, xvilaca, ler\}@tecnico.ulisboa.pt
	}
	
	\IEEEauthorblockA{ 
		\IEEEauthorrefmark{2}
		Department of Computer Architecture, Universitat Polit\`{e}cnica de Catalunya. Barcelona, Spain
		\\\{mkhan, felix\}@ac.upc.edu
	}
} 

